Robust Domain Randomised Reinforcement Learning through Peer-to-Peer Distillation

In reinforcement learning, domain randomisation is an increasingly popular technique for learning more general policies that are robust to domain-shifts at deployment. However, naively aggregating information from randomised domains may lead to high variance in gradient estimation and unstable learning process. To address this issue, we present a peer-to-peer online distillation strategy for RL termed P2PDRL, where multiple workers are each assigned to a different environment, and exchange knowledge through mutual regularisation based on Kullback-Leibler divergence. Our experiments on continuous control tasks show that P2PDRL enables robust learning across a wider randomisation distribution than baselines, and more robust generalisation to new environments at testing.

==> sec4/table_figure2.tex <==
\begin{figure}[t]

\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/train_lc/walker-v2.pdf}
    \caption{Training return on Walker}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/train_lc/Ant-v2.pdf}
    \caption{Training return on Ant}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/train_lc/Humanoid-v2.pdf}
    \caption{Training return on Humanoid }
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/train_lc/Hopper-v2.pdf}
    \caption{Training return on Hopper}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/train_lc/HalfCheetah-v2.pdf}
    \caption{Training return on HalfCheetah}
\end{subfigure}

% train
%
% test

\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/gene_performance/Walker2d-v2.pdf}
    \caption{Testing return on Walker}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/gene_performance/Ant-v2.pdf}
    \caption{Testing return on Ant}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/gene_performance/Humanoid-v2.pdf}
    \caption{Testing return on Humanoid}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/gene_performance/Hopper-v2.pdf}
    \caption{Testing return on Hopper}
\end{subfigure}
\begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width = \textwidth]{figure/gene_performance/HalfCheetah-v2.pdf}
    \caption{Testing return on HalfCheetah}
\end{subfigure}
\caption{Summary of training and generalisation performances across five different continuous control tasks. The leftmost column illustrate the task. The middle column compares the learning performance, represented by learning curves. The rightmost column shows the testing performance as a function of randomised distribution diversity $x$. All experiments are trained with a predefined distribution at $x=0.2$. Results are averaged over 8 different random seeds.\cut{\textcolor{magenta}{How does train distribution variance (and mean) relate to test distribution variance here?}}}
\label{fig: table fig}
\end{figure}

% Middle column: X: Iterations, Y: Return.
% Right: X: Domain parameter. Or width of domain parameter.

==> tmp_subsection.tex <==
\subsection{Further Analysis}

The prior experiments train the peers with the identical distribution of domains. In this experiments, we explore the impact partitioning the domain distribution on learning performance. Specifically, for Walker and Ant tasks, we manually partition the wind condition into two clusters, one with positive wind and the other with negative. As shown in Fig.~\ref{fig: partition}, partitioning the training distribution does not leads to significant difference comparing to learning with one single unified distribution. 
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{figure/ws/Walker2d-v2_partition.pdf}
    \caption{Walker task training }
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{figure/ws/Walker2d-v2_partition_gene.pdf}
    \caption{Walker task testing}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{figure/ws/Ant-v2_partition.pdf}
    \caption{Ant task training}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
    \includegraphics[width=\textwidth]{figure/ws/Ant-v2_partition_gene.pdf}
    \caption{Ant task testing}
    \end{subfigure}
    % \includegraphics{}
    \caption{Comparison between learning with an unified domain and learning with two partitions in Walker task (a,b) and Ant task (c,d).}
    \label{fig: partition}
\end{figure}

